SeqL: Secure Scan-Locking for IP Protection

Existing logic-locking attacks are known to successfully decrypt functionally correct key of a locked combinational circuit. It is possible to extend these attacks to real-world Silicon-based Intellectual Properties (IPs, which are sequential circuits) through scan-chains by selectively initializing the combinational logic and analyzing the responses. In this paper, we propose SeqL, which achieves functional isolation and locks selective flip-flop functional-input/scan-output pairs, thus rendering the decrypted key functionally incorrect. We conduct a formal study of the scan-locking problem and demonstrate automating our proposed defense on any given IP. We show that SeqL hides functionally correct keys from the attacker, thereby increasing the likelihood of the decrypted key being functionally incorrect. When tested on pipelined combinational benchmarks (ISCAS,MCNC), sequential benchmarks (ITC) and a fully-fledged RISC-V CPU, SeqL gave 100% resilience to a broad range of state-of-the-art attacks including SAT[1], Double-DIP[2], HackTest[3], SMT[4], FALL[5], Shift-and-Leak[6] and Multi-cycle attacks[7].

==> backup_results.tex <==
%\begin{table}[!htbp]
%\begin{center}
%\caption{Resilience of {\em SeqL} for Sequential Benchmarks. The locking is done using {\em IBLA} algorithm.}%\label{tab:results-proposed-eff-sequential}
%\begin{tabular}{|c|c|c|c|c|c|c|c|}
%%\hline
%	  & \multicolumn{3}{c|}{{\em EFF}~\cite{rajit:encryptFF}} & \multicolumn{4}{c|}{{\em SeqL}} \\
%\hline
%	Bench.  & Res. & RT	& Ov.			  & Res. & RT & $|K_{ppo}|$ & $\gamma$ \\
%\hline
%\texttt{b01} & \redx & 0.01s & 9.1\% & \greencheck & 0.01s &4 & 20\% \\
%\hline
%\texttt{b02} & \redx & 0.01s & 11.8\%  & \greencheck & 0.01s &3 & 20 \% \\
%\hline
%\texttt{b03} & \redx & 2.1s & 14.2\%   & \greencheck & 4.4s & 5 & 20 \% \\
%\hline
%\texttt{b04} & \redx & 52.4s & 7.8\%   & \greencheck & 56.6s & 4 & 10 \%  \\
%\hline
%%\texttt{b05} & \redx & 8.2s & 3.3\%   & \greencheck & 15.0s & 3 & 5\% \\
%\hline
%\texttt{b06} & \redx & 0.01s & 13.6\%   &  \greencheck & 0.1s & 2 & 20 \% \\
%\hline
%\texttt{b07} & \redx & 30.6s & 9.3\%   & \greencheck & 38.3s & 3 & 10 \% \\
%\hline
%\texttt{b08} & \redx & 0.49s & 9.9\%   &\greencheck & 1.5s & 3 & 15\%  \\
%\hline
%\texttt{b09} & \redx & 0.93s & 12.5\%   & \greencheck & 0.95s & 2 & 15 \%  \\
%\hline
%\texttt{b10} & \redx & 0.31s & 7.6\%   & \greencheck & 0.5s & 3 & 10\%  \\
%\hline
%\texttt{b11} & \redx & 5.47s & 3.8\%   & \greencheck & 9.5s & 2 & 5\%  \\
%\hline
%\texttt{b12} & \redx & 66.6s & 9.3\%   & \greencheck & 163s& 2 & 10\%  \\
%\hline
%\texttt{b13} & \redx & 24.1s & 11.8\%   & \greencheck & 36.9s & 4 & 15\%  \\
%\hline
%\texttt{b14} & \redx & 109.4s & 1.0\%   & \greencheck & $\approx 14 m$ & 8 & 1\%  \\
%\hline
%\texttt{b15} & \redx & 78.8s &0.7\%   & \greencheck & $\approx 35 m$ & 9 & 1\%  \\
%\hline
%\texttt{b17} & \redx & 187s &0.3\%   & \greencheck & $\approx 37 m$ & 16 & 0.5\%  \\
%\hline 
%%\texttt{b18} & \redx & $\approx 521 min$ &0.08\%   & & & 5&  0.09\%\\
%%\hline
%%\texttt{b19} & & &2.6\%   & & & &2.7\%  \\
%%\hline
%%\texttt{b20} & \redx & 257s & 0.5\%   & &   & 5 &0.5\%   \\
%%\hline
%%\texttt{b21}& & &2.2\%   & & & &2.2\%  \\
%%\hline
%%\texttt{b22} & & &2.9\%   & & & &2.3\%  \\
%%\hline
%%Success & \% & - &  - & \% & - & - & -\\
%%\hline
%%\hline
%%\texttt{s27}  & \redx & 0.002s & 31.8 \% & \greencheck& 0.01s & 3 & 34 \% \\
%%\hline 
%%\texttt{s208}  & \redx & 0.009s &  4.8\% & \greencheck& 0.05 & 2 & 7\%\\
%%\hline 
%%\texttt{s298}  & \redx & 0.49s &  4.5\% & \greencheck& 1.8s & 1 & 5.1 \%\\
%%\hline
%%\texttt{s344}  & \redx & 0.016s &  3.8\% & \greencheck& 0.06s & 2 & 4.7\%\\
%%\hline
%%\texttt{s349}  & \redx & 0.017s &  3.7\% & \greencheck& 0.13s & 3 & 5.2 \%\\
%%\hline
%%%%%%%%%%%%%%%%%%\texttt{s382}  & \redx & 0.35s &  4.2\% & \greencheck& 3.2s & 2 & 5 \%\\
%%\hline
%%\texttt{s386}  & \redx & 0.019s &  3.0\% & \greencheck& 0.1s & 3 & 5.8 \%\\
%%\hline
%%\texttt{s400}  & \redx & 0.39s &  4.2\% & \greencheck& 0.96s & 2 & 4.9\%\\
%%\hline
%%\texttt{s420}  & \redx & 0.017s &  3.4\% & \greencheck & 0.1s & 2 & 4.2 \% \\
%%\hline
%%\texttt{s444} & \redx & 0.29s &  3.3\% & \greencheck& 0.67s& 2 & 3.9\%\\
%%\hline
%%\texttt{s510}  & \redx & 0.02s &  2.4\% & \greencheck& 0.06s& 3& 5.7\%\\
%%\hline
%%\texttt{s526}  & \redx & 0.14s &  3.2\% & \greencheck& 1.2s & 4& 15.0 \%\\
%%\hline
%%\texttt{s641}   & \redx & 0.03s &  2.5\% & \greencheck& 0.18s & 2 & 6.1\%\\
%%\hline
%%\texttt{s713} & \redx & 0.03s &  2.5\% & & & & \\
%%\hline
%\texttt{s820} & \redx & 0.03s &  1.6\% & & & %& \\
%%\hline
%%\texttt{s832}  & \redx & 0.04s &  1.6\% & & & & \\
%%\hline
%%\texttt{s838}  & \redx & 0.05s &  2.2\% & & & & \\
%%\hline
%%\texttt{s953}  & \redx & 0.18s &  2.3\% & & & & \\
%%\hline
%%\texttt{s1196}  & \redx & 0.05s &  2.1\% & & & & \\
%%\hline
%%\texttt{s1238}  & \redx & 0.05s &  2.1\% & & & & \\
%%\hline
%%\texttt{s1423}  & \redx & 4.51s &  1.2\% & & & & \\
%%\hline
%%\texttt{s1488}  & \redx & 0.06s &  0.9\% & & & & \\
%%\hline
%%\texttt{s1494}  & \redx & 0.06s &  0.9\% & & & & \\
%%\hline
%%\texttt{s5378}  & & & & & & & \\
%%\hline
%%\texttt{s9234}  & \redx & 128s &  0.4\% & \greencheck & $\approx 4hrs.$ & 9 & 0.45 \%\\
%%\hline
%%\texttt{s13207}  & & & & & & & \\
%%\hline
%%\texttt{s15850}  & & & & & & & \\
%%\hline
%%\texttt{s35932}  & & & & & & & \\
%%\hline
%%\texttt{s38417}  & & & & & & & \\
%%\hline
%%\texttt{s38584}  & & & & & & & \\
%%\hline
%\end{tabular}
%\end{center}
%\end{table}

%\begin{table*}[!t]
%\begin{center}
%\caption{Resilience of {\em SeqL} against other state-of-the-art attacks on pipelined combinational benchmarks. The FO locking is done using {\em IKPA} algorithm.}
%\label{tab:results-proposed-eff-c}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
%\hline
%Bench. & \multicolumn{3}{c|}{SAT~\cite{pramod:host15}} & \multicolumn{3}{c|}{HackTest~\cite{hacktest}} & \multicolumn{2}{c|}{FALL~\cite{pramod-faa}} \\
%\hline
%	& {\em SARLock}~\cite{SARLock}  & {\em TTLock}~\cite{TTLock} & {\em SFLL}~\cite{SFLL} &
%	{\em SARLock}~\cite{SARLock}  & {\em TTLock}~\cite{TTLock} & {\em SFLL}~\cite{SFLL} & 
%	 {\em TTLock}~\cite{TTLock} & {\em SFLL}~\cite{SFLL}   \\

%\hline 
%\texttt{apex2}      
%& &\bluecheck &\bluecheck & &\bluecheck &\bluecheck &\bluecheck &\color{red}{No-key} \\

%\hline  
%\texttt{apex4}   
%& &\bluecheck &\bluecheck & &\bluecheck &\bluecheck & \color{red}{No-key} & \bluecheck \\

%\hline 
%\texttt{i4}       
%& &\bluecheck &\bluecheck & &\bluecheck &\bluecheck &\bluecheck & \\

%\hline 
%\texttt{i7}      
%& &\bluecheck &\bluecheck & &\bluecheck    & &\bluecheck & \\

%\hline 
%\texttt{i8}
%& &\bluecheck &\bluecheck & &\bluecheck &\bluecheck &\bluecheck & \\

%\hline 
%\texttt{i9}     	
%& &\bluecheck & & &\bluecheck & &\bluecheck & \\

%\hline 
%\texttt{seq}     
%& &\color{red}{$>$ abort-limit} & & &\color{red}{$>$ abort-limit} & &\bluecheck & \\

%\hline 
%\texttt{k2}     
%& &\bluecheck & & &\bluecheck & &\bluecheck &\bluecheck \\

%%\hline 
%%\texttt{ex5}     
%%& & & & & & & & \\

%\hline 
%\texttt{ex1010}  
%& &\bluecheck & & &\bluecheck & & \color{red}{No-key} & \\

%\hline
%\texttt{dalu}    
%& &\bluecheck & & &\bluecheck & &\bluecheck & \\

%\hline 
%\texttt{des}     
%& &\bluecheck & & &\bluecheck & &\bluecheck & \\

%\hline 
%\texttt{c432}   
%& &\bluecheck & & &\bluecheck & &\bluecheck &  \\

%\hline 
%\texttt{c499}    
%& &\bluecheck & & &\bluecheck & &\bluecheck &\bluecheck \\

%\hline 
%\texttt{c880}    
%& &\bluecheck  & & &\bluecheck & &\bluecheck & \\

%\hline 
%\texttt{c1355}   
%& &\bluecheck & & &\bluecheck & &\bluecheck & \\

%\hline
%\texttt{c1908}   
%& &\bluecheck & & &\bluecheck & &\bluecheck & \\

%\hline 
%\texttt{c3540}   
%& &\bluecheck & & &\bluecheck & &\bluecheck & \\

%\hline 
%\texttt{c5315}   
%& &\color{red}{$>$ abort-limit} & & &\color{red}{$>$ abort-limit} & &\bluecheck & \\

%\hline 
%\texttt{c7552}   
%& &\bluecheck & & &\bluecheck & &\bluecheck & \\

%\hline 
%%\hline 
%\end{tabular}
%\end{center}
%\end{table*}

%\begin{table}[!t]
%\begin{center}
%\caption{Resilience of {\em SeqL} to oracle-less attacks}
%\vspace{-1em}
%\label{tab:results-seql-}
%\begin{tabular}{|c|c|c|c|}
%\hline
%	Bench.  &
%	Removal-attack~\cite{removal-attack} & HackTest~\cite{hacktest}
%	 & FALL~\cite{pramod-faa} \\
%\hline
%\texttt{b01}  & \bluecheck  & \bluecheck & \\
%\hline
%\texttt{b02}  & \bluecheck & \bluecheck & \\
%\hline
%\texttt{b03} & \bluecheck & \bluecheck &  \\
%\hline
%\texttt{b04} & \bluecheck  & \bluecheck & \\
%\hline
%\texttt{b05} & \bluecheck  & \bluecheck &  \\
%\hline
%\texttt{b06} & \bluecheck & \bluecheck & \\
%\hline
%\texttt{b07} & \bluecheck & \bluecheck & \\
%\hline
%\texttt{b08} & \bluecheck & \bluecheck &  \\
%\hline
%\texttt{b09} & \bluecheck & \bluecheck &  \\
%\hline
%\texttt{b10} & \bluecheck & \bluecheck &  \\
%\hline
%\texttt{b11} & \bluecheck & \bluecheck & \\
%\hline
%\texttt{b12} & \bluecheck & \bluecheck &  \\
%\hline
%\texttt{b13} & \bluecheck & \bluecheck &  \\
%\hline
%\texttt{b14} & \bluecheck & \bluecheck &  \\
%\hline
%\texttt{b15} & \bluecheck & \bluecheck &  \\
%\hline
%\texttt{b17} & \bluecheck & %\bluecheck &  \\
%\hline
%\texttt{b18} & \bluecheck &  & \bluecheck & \bluecheck &   &\\
%\hline
%\texttt{b19} & \bluecheck &  & \bluecheck & \bluecheck &   &\\
%\hline
%\texttt{b20} & \bluecheck &  & \bluecheck & \bluecheck &   &\\
%\hline
%\texttt{b21} & \bluecheck &  & \bluecheck & \bluecheck &   &\\
%\hline
%\texttt{b22} & \bluecheck &  & \bluecheck & \bluecheck &   &\\
%\hline
%\end{tabular}
%\end{center}
%\vspace{-2em}
%\end{table}





%\subsection{Decryption time}
%Comparison of decryption times for ITC'99 circuits were shown earlier in Figure~\ref{tab:results-proposed-eff-sequential}. Figure~\ref{fig:rt-comparison-seql-eff} shows the comparison of key decryption times of {\em SeqL} (red) with {\em EFF} (blue) techniques for pipelined combinational benchmarks, on the 4 different encryption schemes validated in~\cite{pramod:host15}. The benchmarks are shown on X-axis and the key decryption time is shown on a logarithmic scale on Y-axis.
%Clearly, {\em SeqL} is superior with regard to decryption time, as compared to {\em EFF}, across all the benchmarks, across all the encryption categories. 
%\begin{figure}[!htbp]
%%\vspace{-0em}
%  \begin{center}
%    \subfigure[RND~\cite{farinaz:epic}]{\label{fig:rnd-rt-comparison}\includegraphics[scale=0.55]{fig/running-time-comparisons-EFF-SeqL-rnd.pdf}}
%    \subfigure[DAC'12~\cite{jv:dac12}]{\label{fig:dac12-rt-comparison}\includegraphics[scale=0.55]{fig/running-time-comparisons-EFF-SeqL-dac12.pdf}}
    %\subfigure[IOLTS'14~\cite{dupuis:iolts14}]{\label{fig:iolts14-rt-comparison}\includegraphics[scale=0.4]{fig/running-time-comparisons-EFF-SeqL-iolts14.pdf}}
%    \subfigure[ToC'13/xor~\cite{jv:tc15}]{\label{fig:toc13xor-rt-comparison}\includegraphics[scale=0.55]{fig/running-time-comparisons-EFF-SeqL-toc13xor.pdf}}
%    \subfigure[ToC'13/mux~\cite{jv:tc15}]{\label{fig:toc13mux-rt-comparison}\includegraphics[scale=0.55]{fig/running-time-comparisons-EFF-SeqL-toc13mux.pdf}}
%  \end{center}
%    \caption{Pipelined combinational benchmarks: key decryption time comparison between {\em SeqL} and {\em EFF}}
%  \label{fig:rt-comparison-seql-eff}
%\end{figure}

%For {\em c7552} (arithmetic benchmark) and {\em des} (cryptographic benchmark), bthere was one or more orders of magnitude increase in decryption time, depending on the encryption category. It is interesting to note that both of these benchmarks inherently have XOR chains in the combinational logic. 
%Thus, in addition to achieving resilience against SAT-attack through functional output corruption, {\em SeqL} also achieves significant increase in decryption time, as compared to {\em EFF}.

\begin{table*}[!htbp]
\begin{center}
\caption{Resilience of {\em SeqL} for ITC'99 Sequential Benchmark Circuits. The Scan-locking was done using {\em IBLA} algorithm. $N$ is number of capture cycles in the multi-cycle scan-test}
%\vspace{-1em}
\label{tab:results-proposed-eff-sequential}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Benchmark	  & \multicolumn{3}{c|}{{\em EFF}~\cite{rajit:encryptFF}} & \multicolumn{11}{|c|}{{\em SeqL}} \\
\hline
     & & & & & & &  \multicolumn{2}{|c|}{$N=1$}    & \multicolumn{2}{|c|}{$N=2$} & \multicolumn{2}{|c|}{$N=3$} & \multicolumn{2}{|c|}{$N=4$}\\
\hline
	  & Res. & Overhead & DT.			  & $n$ & $p$& $\gamma$ & Res. & DT. & Res.  & DT. &  Res. & DT. &  Res. & DT.\\
\hline
\texttt{b01} & \redx & $9$\% & $10ms$ & $4$ & $0.93$& $20$\%  & \bluecheck & $10ms$ &\bluecheck &$10ms$ & & & &\\
\hline                                 
\texttt{b02} & \redx & $12$\%  & $10ms$ &$3$ & $0.88$& $20$ \%  & \bluecheck & $10ms$ & & & & & &\\
\hline
\texttt{b03} & \redx & $14$\%   & $2.1s$& $5$ & $0.97$& $20$ \%  & \bluecheck & $4.4s$ & & & & & &\\
\hline
\texttt{b04} & \redx & $8$\%   & $52s$ & $4$ & $0.93$& $10$ \%   & \bluecheck & $57s$ & & & & & &\\
\hline
\texttt{b05} & \redx & $3$\%   & $8.2$s & 3 & $0.88$& $5$\%  & \bluecheck & $15$s & & & & & &\\
\hline
\texttt{b06} & \redx & $14$\%   & $10ms$ & $2$ & $0.75$& $20$ \%  & \bluecheck & $0.1s$ & & & & & &\\
\hline
\texttt{b07} & \redx & $9$\%   & $31s$ & $3$ & $0.88$& $10$ \%  & \bluecheck & $38s$ & & & & & &\\
\hline
\texttt{b08} & \redx & $10$\%   & $0.5s$ & 3 & $0.88$& 15\%  & \bluecheck & $1.5s$ & & & & & &\\
\hline
\texttt{b09} & \redx & $13$\%   & $0.9s$ & 2 & $0.75$& 15 \%   & \bluecheck & $1.0s$ & & & & & &\\
\hline
\texttt{b10} & \redx & $8$\%   & $0.3s$ & 3 & $0.88$& 10\%   & \bluecheck & $0.5$ & & & & & &\\
\hline
\texttt{b11} & \redx & $4$\%   & $5.5s$ & 2 & $0.75$& 5\%  & \bluecheck & $9.5s$ & & & & & &\\
\hline
\texttt{b12} & \redx & $10$\%   & $67s$ & 2 & $0.75$& 10\%   & \bluecheck & $163s$ & & & & & &\\
\hline
\texttt{b13} & \redx & $12$\%   & $24s$ & 4 & $0.93$& 15\%   & \bluecheck & $37s$ & & & & & &\\
\hline
\texttt{b14} & \redx & $1.0$\%   & $109s$ & 8 & $0.99$& 1\%   & \bluecheck & $ 14m$ & & & & & &\\
\hline
\texttt{b15} & \redx &$0.7$\%   & $79s$ & 9 & $0.99$& 1\%   & \bluecheck & $ 35m$ & & & & & &\\
\hline
\texttt{b17} & \redx &$0.3$\%   & $187s$ & 16 & $0.99$& 0.5\%   & \bluecheck & $ 37m$ & & & & & &\\
\hline 
\end{tabular}
\end{center}
%\vspace{-2em}
\end{table*}


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\subsection{Comparison to Timing-Driven SAT Defenses}
\label{sec:genericness}
In~\cite{delay-locking}, {\em delay-locking} was proposed to mitigate SAT-attack. In {\em delay-locking}, the key not only determines the functionality of the circuit but also its timing profile. A functionally-correct but timing-incorrect key will result in timing violations and thus make the circuit malfunction. In~\cite{TimingSAT}, a novel SAT formulation based approach called {\em TimingSAT} was used to deobfuscate the functionalities of such delay locked designs within a reasonable amount of time. Since delay locking is orthogonal to {\em EFF} in defending SAT-attack, we do not compare with {\em delay-locking} or {\em TimingSAT}.

\subsection{Cyclic Obfuscation}
\label{sec:cyc-obfuscation}
The verification effort involved for \emph{cyclic combinational circuits} does not scale well for complex designs~\cite{cyclic-verification}, hence cyclic logic obfuscation is arguably impractical to industry.  We therefore did not compare against this class of techniques in this paper. 

\subsection{Scan compression}
\label{sec:compression}
So far, we have discussed scan-based attacks in the bypass mode, and not through the compression hardware. The ScanSAT~\cite{lilas:aspdac19} addresses launching attack in compression mode, but their results are restricted to XOR-based compression and do not consider EDT. Although EDT is industry standard for scan-compression, none of the existing works look at launching the attacks in EDT-mode. 
%It is well known that industrial circuits have test cubes with $\>97\%$ X-bits~\cite{edt}, EDT exploits this property to efficiently decompress test patterns. Thus, EDT expects X-bits in its test cubes, which is contradictory to existing logic locking attacks, which expect full control over the test cubes, thereby intuitively provides natural resilience to logic locking attacks. 
In~\cite{guin:2018}, they discuss the resilience of compressor to logic locking attacks. However, there is no work so far on resilience of EDT decompressor. The EDT decompressor is composed of ring generator and phase shifter, which operate on {\em Galois fields} to produce the test vectors. Quantifying the natural resilience of decompressor to oracle-guided attacks and intelligent decompressor design to resist these attacks, is an open problem. 

%\subsection{Split Manufacturing}
%\label{sec:sm}
%Split-manufacturing has been an orthogonally researched topic.  Split-manufacturing is actively being researched by Intelligence Advanced Research Projects Activity (IARPA) Trusted Integrated Chips (TIC)  Program for IP protection~\cite{iarpa-split-manufacturing}. 

%\subsection{Limitations of SeqL}
%\label{sec:limitations}
%While  {\em ScanSAT}~\cite{lilas:aspdac19} uses {\em EFF} as a representative example, there are other scan-locking variants. While {\em EFF} uses statically obfuscated scan-chains, a dynamically-obfuscated-scan (DOS) architecture is proposed in~\cite{wang:2017} and design-for-security (DFS) architecture is proposed in~\cite{guin:2018}. Recently, shift-and-leak~\cite{shift-and-leak-iccad19} attack was proposed that is able to decrypt about $95\%$ of the encryption key in the presence of scan-locking technique proposed in~\cite{guin:2018}. We do not cover those extensions in this work.

%From Table~\ref{tab:results-proposed-eff-sequential}, we note that value of $n=|K_{fi}| = |K_{sq}|$ in most cases is less than $10$. So, the total number of possible sequential key bits is $ |K_{fi}| + |K_{sq}|< 20$, hence it is possible to find the functionally correct key using brute-force-search. Solution to address this issue is to lock extra FOs (after Algorithm~\ref{alg:ipla-c-pipelined} or~\ref{alg:ibla} quits), which results in exponential increase in sequential key search space, with linear increase in area overhead.    

==> results_old.tex <==
\begin{table*}[!htbp]
\begin{center}
\caption{Resilience of {\em SeqL} for ITC'99 Sequential Benchmark Circuits. The FO locking was done using {\em IBLA} algorithm. $N$ is number of capture cycles in the multi-cycle scan-test}
%\vspace{-1em}
\label{tab:results-proposed-eff-sequential}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Benchmark	  & \multicolumn{3}{c|}{{\em EFF}~\cite{rajit:encryptFF}} & \multicolumn{11}{|c|}{{\em SeqL}} \\
\hline
     & & & & & & &  \multicolumn{2}{|c|}{$N=1$}    & \multicolumn{2}{|c|}{$N=2$} & \multicolumn{2}{|c|}{$N=3$} & \multicolumn{2}{|c|}{$N=4$}\\
\hline
	  & Res. & Overhead & DT.			  & $n$ & $p$& $\gamma$ & Res. & DT. & Res.  & DT. &  Res. & DT. &  Res. & DT.\\
\hline
\texttt{b01} & \redx & $9$\% & $10ms$ & $4$ & $0.93$& $20$\%  & \bluecheck & $10ms$ & & & & & &\\
\hline                                 
\texttt{b02} & \redx & $12$\%  & $10ms$ &$3$ & $0.88$& $20$ \%  & \bluecheck & $10ms$ & & & & & &\\
\hline
\texttt{b03} & \redx & $14$\%   & $2.1s$& $5$ & $0.97$& $20$ \%  & \bluecheck & $4.4s$ & & & & & &\\
\hline
\texttt{b04} & \redx & $8$\%   & $52s$ & $4$ & $0.93$& $10$ \%   & \bluecheck & $57s$ & & & & & &\\
\hline
\texttt{b05} & \redx & $3$\%   & $8.2$s & 3 & $0.88$& $5$\%  & \bluecheck & $15$s & & & & & &\\
\hline
\texttt{b06} & \redx & $14$\%   & $10ms$ & $2$ & $0.75$& $20$ \%  & \bluecheck & $0.1s$ & & & & & &\\
\hline
\texttt{b07} & \redx & $9$\%   & $31s$ & $3$ & $0.88$& $10$ \%  & \bluecheck & $38s$ & & & & & &\\
\hline
\texttt{b08} & \redx & $10$\%   & $0.5s$ & 3 & $0.88$& 15\%  & \bluecheck & $1.5s$ & & & & & &\\
\hline
\texttt{b09} & \redx & $13$\%   & $0.9s$ & 2 & $0.75$& 15 \%   & \bluecheck & $1.0s$ & & & & & &\\
\hline
\texttt{b10} & \redx & $8$\%   & $0.3s$ & 3 & $0.88$& 10\%   & \bluecheck & $0.5$ & & & & & &\\
\hline
\texttt{b11} & \redx & $4$\%   & $5.5s$ & 2 & $0.75$& 5\%  & \bluecheck & $9.5s$ & & & & & &\\
\hline
\texttt{b12} & \redx & $10$\%   & $67s$ & 2 & $0.75$& 10\%   & \bluecheck & $163s$ & & & & & &\\
\hline
\texttt{b13} & \redx & $12$\%   & $24s$ & 4 & $0.93$& 15\%   & \bluecheck & $37s$ & & & & & &\\
\hline
\texttt{b14} & \redx & $1.0$\%   & $109s$ & 8 & $0.99$& 1\%   & \bluecheck & $ 14m$ & & & & & &\\
\hline
\texttt{b15} & \redx &$0.7$\%   & $79s$ & 9 & $0.99$& 1\%   & \bluecheck & $ 35m$ & & & & & &\\
\hline
\texttt{b17} & \redx &$0.3$\%   & $187s$ & 16 & $0.99$& 0.5\%   & \bluecheck & $ 37m$ & & & & & &\\
\hline 
\end{tabular}
\end{center}
%\vspace{-2em}
\end{table*}


\section{Experimental Evaluation}
\label{sec:results}

\noindent We validate the security of {\em SeqL} against a multitude of state-of-the-art attacks and quantify its reduced overheads compared to prior work. This analysis confirms our claims on genericness, robustness, and scalability of {\em SeqL}.



In order to perform {\em ScanSAT} resilience evaluation, we have used {\em sld} key generation solver and {\em lcmp} formal-equivalence checkers provided by~\cite{pramod:host15}. Both the solvers use the {\em .bench} format for the input benchmark circuit. In all the subsequent experiments, we have used the open-source {\em .bench} designs for ITC'99 sequential benchmarks available at~\cite{itc99} and logic-encrypted ISCAS'85, MCNC combinational benchmarks provided by~\cite{pramod:host15}. 
Algorithms~\ref{alg:ibla} ({\em IBLA}) and~\ref{alg:ipla-c-pipelined} were used for sequentially locking the sequential benchmarks and pipelined combinational benchmarks, respectively. Both the locking algorithm were implemented in {\em Perl}. Since the locking algorithm execution times across all the benchmarks is very small (matter of seconds), the execution times were not reported.  

Table~\ref{tab:results-proposed-eff-sequential} shows the results of applying the procedure shown in Figure~\ref{fig:flowchart} on ITC'99 sequential circuits. The columns {\em Res.}, {\em Ov.} and {\em DT} indicate overhead and decryption time respectively. The resilience rate of {\em EFF} was 0\%, while that of {\em SeqL} was 100\%, thus indicating the superiority of  {\em SeqL} over {\em EFF}. An abort limit of $24 hours$ was used for key decryption. The key decryption time for \texttt{b18} and \texttt{b19} circuits was more than this abort limit, without any result, hence the results for these 2 benchmarks are not reported. 



\begin{table}[!t]
\begin{center}
\caption{Resilience of {\em SeqL} for Pipelined Combinational Benchmarks for $5\%$ logic encryption. The FO locking is done using {\em IKPA} algorithm.}
\label{tab:results-proposed-eff-c}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Bench. & \multicolumn{2}{c|}{RND} & \multicolumn{2}{c|}{DAC'12} & \multicolumn{2}{c|}{ToC'13/xor} & \multicolumn{2}{c|}{ToC'13/mux} \\
\hline
	& {\em EFF}  & {\em SeqL} &
	{\em EFF} & {\em SeqL} & 
	{\em EFF} & {\em SeqL} & 
	{\em EFF} & {\em SeqL}  \\
%\hline
%       &~\cite{dupuis:iolts14}  & $P_1$  & $P_2$ &~\cite{dupuis:iolts14}  & $P_1$ & $P_2$ &~\cite{dupuis:iolts14}  & $P_1$ & $P_2$ &~\cite{dupuis:iolts14}  & $P_1$ & $P_2$ &~\cite{dupuis:iolts14}  & $P_1$ & $P_2$  \\

\hline 
\texttt{apex2}      
&\redx	&\bluecheck		&\redx &\bluecheck			%&\redx &\greencheck 		
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline  
\texttt{apex4}   
&\redx	&\bluecheck			&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\bluecheck &\bluecheck \\

\hline 
\texttt{i4}       
&\bluecheck &\bluecheck 		&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline 
\texttt{i7}      
&\bluecheck &\bluecheck 		&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline 
\texttt{i8}     	&\bluecheck &\bluecheck		&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline 
\texttt{i9}     	&\bluecheck &\bluecheck		&\redx &\bluecheck		%&\redx &\greencheck 	
&\redx &\bluecheck				&\redx &\bluecheck \\

\hline 
\texttt{seq}     
&\bluecheck & \bluecheck		&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline 
\texttt{k2}     	&\bluecheck &\bluecheck		&\redx &\bluecheck		%&\redx &\greencheck	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline 
\texttt{ex5}     
&\bluecheck &\bluecheck		&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline 
ex1010  
&\bluecheck &\bluecheck 		&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline
\texttt{dalu}    
&\bluecheck	&\bluecheck	&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline 
\texttt{des}     
&\bluecheck &\bluecheck 		&\redx &\bluecheck	%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline 
\texttt{c432}   
&\redx &\bluecheck			&\redx &\bluecheck		%&\redx &\greencheck  	
&\redx &\bluecheck 			&\redx &\bluecheck  \\

\hline 
\texttt{c499}    
&\redx &\bluecheck 			&\redx &\bluecheck 		%&\redx &\greencheck 	
&\redx &\bluecheck				&\redx &\bluecheck \\

\hline 
\texttt{c880}    
&\bluecheck	&\bluecheck	&\bluecheck &\bluecheck	%&\redx &\greencheck 	
&\redx &\bluecheck			&\redx &\bluecheck \\

\hline 
\texttt{c1355}   
&\bluecheck &\bluecheck		&\redx &\bluecheck		%&\redx &\greencheck 	
&\bluecheck &\bluecheck		&\redx &\bluecheck \\

\hline
\texttt{c1908}   
&\bluecheck &\bluecheck		&\redx &\bluecheck		%&\redx &\greencheck 	
&\redx &\bluecheck 			&\redx &\bluecheck \\

\hline 
\texttt{c3540}   &\bluecheck &\bluecheck 		&\redx &\bluecheck		&\redx %&\greencheck	&\redx 
&\bluecheck				&\redx &\bluecheck \\

\hline 
\texttt{c5315}   &\bluecheck &\bluecheck		&\bluecheck &\bluecheck	&\redx %&\greencheck 	&\greencheck 
&\bluecheck			&\redx &\bluecheck \\

\hline 
\texttt{c7552}   &\bluecheck &\bluecheck		&\redx &\bluecheck		&\redx %&\greencheck 	&\greencheck 
&\bluecheck			&\redx &\bluecheck \\

\hline 
%c2670  &\greencheck &\greencheck		&- &-		&\redx &\greencheck	& &\greencheck &\greencheck 			&\redx &\greencheck \\
%\hline 
%Success  &$80\%$ &$100\%$			&$10\%$ &$100\%$			&$0\%$ &$100\%$ 		&$70\%$ &$100\%$				&$5\%$ &$100\%$ \\
%\hline 
\end{tabular}
\end{center}
\end{table}


Table~\ref{tab:results-proposed-eff-c} shows the results of applying the procedure shown in Figure~\ref{fig:flowchart} on 4 different encryption schemes validated in~\cite{pramod:host15}, and compared against {\em EFF}~\cite{rajit:encryptFF}. 
%Due to shortage of space, the proposed technique is shown in column labeled {\em P} and {\em EFF} is referred to its citation. 
This table shows that {\em SeqL} secured all sequential circuits against {\em ScanSAT} in $100 \%$ of the cases.  As explained in Section~\ref{sec:insight}, 
\begin{itemize}
    \item $K_c$ was successfully decrypted in all cases, while 
    \item $K_{fi}$ and $K_{fo}$ were incorrect, hence causing functional output corruption, thus achieving resilience.
\end{itemize}
Results on $IOLTS'14$ gave 0\% resilience in {\em EFF} case and 100\% resilience in {\em SeqL} case, across all benchmarks, hence not reported in Table~\ref{tab:results-proposed-eff-c} for shortage of space. On the other hand, results on $DTC'10/LUT$ were not reported because it is LUT-based. 

\subsection{Multi-cycle tests}
\label{sec:multi-cycle-tests}
So far, we have discussed the attack in the context of a 1-cycle test. It is possible that the attacker uses the scan-chain to import the input vectors, runs the circuit for more than 1 cycle (multi-cycle test), and observe the output through the scan-chain. Even for such multi-cycle tests, {\em SeqL} can still defend SAT-attack, since the functional isolation is still applicable during scanning-in input vectors and scanning-out the responses.


\begin{table}[!htbp]
\begin{center}
\caption{Resilience of {\em SeqL} $+$ TTLock~\cite{TTLock} against state-of-the-art attacks on pipelined combinational benchmarks.} 
\label{tab:results-sota-attacks}
\begin{tabular}{|c|c|c|c|}
\hline
Bench. & HackTest~\cite{hacktest} & ScanSAT~\cite{lilas:aspdac19} & FALL~\cite{pramod-faa} \\

 & (2017) & (2019) & (2019) \\
\hline 
\texttt{apex2}      
&\bluecheck &\bluecheck &\bluecheck \\

\hline  
\texttt{apex4}   
&\bluecheck &\bluecheck & \color{red}{{\bf No-key}} \\

\hline 
\texttt{i4}       
&\bluecheck &\bluecheck &\bluecheck \\

\hline 
\texttt{i7}      
&\bluecheck &\bluecheck &\bluecheck \\

\hline 
\texttt{i8}
&\bluecheck &\bluecheck &\bluecheck\\

\hline 
\texttt{i9}     	
&\bluecheck &\bluecheck &\bluecheck\\

\hline 
\texttt{seq}     
&\color{red}{$>$ {\bf abort-limit}} &\color{red}{$>$ {\bf abort-limit}}  &\bluecheck \\

\hline 
\texttt{k2}     
&\bluecheck &\bluecheck &\bluecheck \\

%\hline 
%\texttt{ex5}     
%& & & & & & & & \\

\hline 
\texttt{ex1010}  
&\bluecheck &\bluecheck & \color{red}{{\bf No-key}} \\

\hline
\texttt{dalu}    
&\bluecheck &\bluecheck &\bluecheck \\

\hline 
\texttt{des}     
&\bluecheck &\bluecheck &\bluecheck \\

\hline 
\texttt{c432}   
&\bluecheck &\bluecheck &\bluecheck  \\

\hline 
\texttt{c499}    
&\bluecheck &\bluecheck &\bluecheck\\

\hline 
\texttt{c880}    
&\bluecheck &\bluecheck &\bluecheck \\

\hline 
\texttt{c1355}   
&\bluecheck &\bluecheck &\bluecheck \\

\hline
\texttt{c1908}   
&\bluecheck &\bluecheck &\bluecheck \\

\hline 
\texttt{c3540}   
&\bluecheck &\bluecheck &\bluecheck \\

\hline 
\texttt{c5315}   
&\bluecheck &\bluecheck &\bluecheck \\
    
\hline 
\texttt{c7552}   
&\bluecheck &\bluecheck &\bluecheck \\

\hline 
%\hline 
\end{tabular}
\end{center}
\end{table}






\subsection{Resilience of scan-unrolled versions of {\em SeqL}-locked design to state-of-the-art attacks on logic locking}
Table~\ref{tab:results-sota-attacks} shows the resilience of {\em SeqL}-locked design to state-of-the-art attacks on logic locking like ScanSAT}~\cite{lilas:aspdac19}, {\em HackTest}-attack~\cite{hacktest} and functional-analysis-attacks on logic-locking (FALL)-attack~\cite{pramod-faa}. The experiments were run on {\bf Henry2} high-performance cluster from North Carolina State University~\cite{henry2}, with an abort-limit of 24 hours. \\

\label{sec:removal-attack}
\noindent {\em \underline{Theorem 4:}} If circuit has $n$ flip-flops, time complexity of removal attack~\cite{removal-attack} is $\mathcal{O}(2^n)$ \\
\indent{\em Proof:} 
 \begin{enumerate}
    \item In the removal attack, the attacker needs to check if each key-gate removed introduces an inversion at the output of flip-flop. Thus, there are $2^n$ possibilities;  
    \item Assuming we use an adjacency list to represent the circuit as $G=(V,E)$, formal equivalence checking of the locked circuit with original circuit, has two steps: graph reduction in terms of decision diagrams and equivalence-checking; 
    \item The graph reduction step is $\mathcal{O}(G.log (G)) = \mathcal{O}(|V+E|.log(|V+E|)})$. Since average-fanout ($|E|/|V|$) and ratio of gates to flip-flops ($|V|/n$) are both upper-bounded,  graph reduction time reduces to $\mathcal{O}(n.log(n))$
    \item It is well-known that combinational-equivalence-checking (CEC) is NP-complete~\cite{bryant:86} (although most practical instances run in polynomial time~\cite{cec:polynomial}). Assume CEC running-time is $O(n^k)$, where $k$ is a complexity constant; 
\end{enumerate}    
Therefore, (even if assuming the NP-complete CEC step takes polynomial running time), the time it takes to launch removal attack is $\mathcal{O}((n.log(n)) + n^k)2^n) = \mathcal{O}(2^n)$, hence the proof.


 

\subsection{Overheads}
\label{sec:overheads}
\noindent Table~\ref{tab:area-timing-energy} shows the comparison of area, timing and energy for original, $EFF$-type and proposed $SeqL$-type locked flip-flops, obtained using SPICE transistor-level simulation. $NGSPICE$ open-source simulator, $Nangate\ 45nm$ library scan flip-flop and $45nm$ predictive technology model was used to arrive at these results. From Table~\ref{tab:area-timing-energy}, it is evident that the proposed $SeqL$-style locked scan flip-flop has $22\%$ and $19\%$ reduction in $T_{CK-to-Q}$ and Energy-Per-Toggle ($EPT$) respectively, with only $4\%$ area overhead as compared to $EFF$-style locked scan flip-flop. 

\begin{table}[!h]
\begin{center}
\caption{Flip-Flops Comparison: Area, Functional Timing and Energy}
\vspace{-0.2in}
\label{tab:area-timing-energy}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
$FF$ & \# Ts  & $T_{setup}$ & $T_{CK-to-Q}$ & \% Inc. &  EPT	 & \% Inc. \\
%	&          &                 &             &               & $T_{CK-to-Q}$  &  ($EPT$)      	 & $EPT$ \\  
\hline
Orig. & $38$ & $45ps$ & $113ps$ & - &  $13.1 fJ$ & - \\
\hline 
$EFF$    & $48$ & $45ps$ & $163ps$ & $44\%$ & $17.1 fJ$ & $31\%$\\
\hline 
$SeqL$   & $50$ & $45ps$ & $127ps$ & $12\%$ & $13.9 fJ$ & $6\%$\\
\hline
\end{tabular}
\end{center}
\end{table}






